VisionLLM: Large Language Model is also an Open-Ended Decoder for Vision-Centric Tasks

Large language models (LLMs) have notably accelerated progress towards artificial general intelligence (AGI), with their impressive zero-shot capacity for user-tailored tasks, endowing them with immense potential across a range of applications. However, in the field of computer vision, despite the availability of numerous powerful vision foundation models (VFMs), they are still restricted to tasks in a pre-defined form, struggling to match the open-ended task capabilities of LLMs. In this work, we present an LLM-based framework for vision-centric tasks, termed VisionLLM. This framework provides a unified perspective for vision and language tasks by treating images as a foreign language and aligning vision-centric tasks with language tasks that can be flexibly defined and managed using language instructions. An LLM-based decoder can then make appropriate predictions based on these instructions for open-ended tasks. Extensive experiments show that the proposed VisionLLM can achieve different levels of task customization through language instructions, from fine-grained object-level to coarse-grained task-level customization, all with good results. It's noteworthy that, with a generalist LLM-based framework, our model can achieve over 60\% mAP on COCO, on par with detection-specific models. We hope this model can set a new baseline for generalist vision and language models. The demo shall be released based on https://github.com/OpenGVLab/InternGPT. The code shall be released at https://github.com/OpenGVLab/VisionLLM.

==> tables/ab_bert.tex <==
\begin{table*}[t]
\centering 
\renewcommand{\arraystretch}{0.95} % Line spacing
\footnotesize

\caption{Ablation on the text encoder in language-guided image tokenizer.}
\setlength\tabcolsep{8pt}
\begin{tabular}{cccc}
        \shline
        w/ BERT & Freeze BERT & COCO & RefCOCO \\
        \hline
        $\times$   & $-$        & $44.7$ & $48.1$ \\
        \checkmark & $\times$   & $44.8$ & $84.1$ \\
        \checkmark & \checkmark & $1.3$ &  $34.3$ \\        
        \shline
\end{tabular}

\label{tab:ab_bert} 
\vspace{-3mm}
\end{table*}
